Self-supervised Speech Models for Word-Level Stuttered Speech Detection

Clinical diagnosis of stuttering requires an assessment by a licensed speech-language pathologist. However, this process is time-consuming and requires clinicians with training and experience in stuttering and fluency disorders. Unfortunately, only a small percentage of speech-language pathologists report being comfortable working with individuals who stutter, which is inadequate to accommodate for the 80 million individuals who stutter worldwide. Developing machine learning models for detecting stuttered speech would enable universal and automated screening for stuttering, enabling speech pathologists to identify and follow up with patients who are most likely to be diagnosed with a stuttering speech disorder. Previous research in this area has predominantly focused on utterance-level detection, which is not sufficient for clinical settings where word-level annotation of stuttering is the norm. In this study, we curated a stuttered speech dataset with word-level annotations and introduced a word-level stuttering speech detection model leveraging self-supervised speech models. Our evaluation demonstrates that our model surpasses previous approaches in word-level stuttering speech detection. Additionally, we conducted an extensive ablation analysis of our method, providing insight into the most important aspects of adapting self-supervised speech models for stuttered speech detection.

==> sections/ablation.tex <==
\subsection{On the selection of Speech SSL Interface}
There are multiple approaches to utilize information from multiple layers of Speech SSL models rather than using Hierarchical Convolution.
In this section we try other alternative methods.
Specifically, we try using weighted sum or simply select a single layer from WavLM (which was done in~\cite{bayerl22b_interspeech,bayerl23_interspeech}.
The results are shown in Table~\ref{tab:Word_level}. 




\subsection{On the effect of Synthetic Stuttering Pretraining}
In this section, we want to investigate the effect of synthetic stuttering pretraining.
Hence, we tried using different scale of the 
% \subsection{On the effect of multitasking with phoneme recognition}
% in \cite{bayerl22b_interspeech}, they show that phoneme recognition and dislfuency mdoel uses the same layers (middle to end) so we want to try if it help

\subsection{On the scale of Fintuning Dataset}

% \subsection{Real or Fake Utterance Level Fintuning Dataset}


==> sections/qualitative.tex <==
\subsection{Visualization of stuttered speech detection}

\subsection{Visualization of Weight Distributions}


